Exploring Privacy Leakage and Data Disclosure Violations in the MacOS Application Ecosystem

The systematic and excessive data collection practices of tech companies have rendered online privacy both a necessity and a sought-after commodity. However, while the privacy risks of the web, mobile, and IoT ecosystems have been extensively examined, desktop environments have been largely overlooked. As desktop apps continue to be widely used, they remain a critical yet understudied dimension of user privacy. In this paper, we address this gap by presenting the first, to our knowledge, comprehensive study of the mechanisms designed to regulate and disclose data collection and sharing practices in the macOS ecosystem. We adopt an app-development-centric view, and shed light on the interactions between the various macOS mechanisms that mediate apps' data access. Driven by our findings, we develop NutriScan, an analysis framework that incorporates both static and dynamic analysis techniques to create a consolidated view of macOS apps' data practices and disclosures. We use our system to dynamically analyze 1K macOS apps, and find that 85% of them access user-data APIs without disclosing it. 49.7% also exfiltrate data to advertising entities and hosting providers, 12.5% of which do so without a corresponding disclosure. We find that desktop apps are being leveraged by online trackers to enrich user profiles and device fingerprints, thus shedding new light on the true scope of the online tracking ecosystem. Our analysis reveals how the macOS app ecosystem is comprised of disjoint mechanisms with divergent data abstractions, thus increasing complexity for developers while also facilitating undisclosed privacy-invasive practices. Accordingly, we propose a series of mitigations that aim to both streamline the data disclosure process for developers and improve Apple's app vetting process.

==> limitations.tex <==

During out testing, we found certain applications which couldn;t be run successfully with Frida hook injection. These applications could be braodly broken into
two categories:

SIP Detection: Some apps query the system runtime environment to detect if SIP is disabled. This can be achieved via csrutil. These can can then refuse to run in an environment where memory integrity can not be verified or proven.
Anti Frida Logic: Some apps detect if Frida was injected in the process by examining the dynamic loading of the process. If they detecta debugger is attached they can modify the functionality

These apps cannot be analyzed via our pipeline. This is drawback of our technique and a direction for future work.


We also provide for SSL pining bypass via the Frida
hooking to capture a wider range of network traffic. Despite
ou best efforts, some application include custom TLS logic
which can be hard to generalize and thus bypass. So a subset
of network requests can’t be intercepted. This is known
drawback which prior researchers have outlined in their
experiments

